Just-in-Time Detection of Silent Security Patches

Open-source code is pervasive. In this setting, embedded vulnerabilities are spreading to downstream software at an alarming rate. While such vulnerabilities are generally identified and addressed rapidly, inconsistent maintenance policies may lead security patches to go unnoticed. Indeed, security patches can be {\em silent}, i.e., they do not always come with comprehensive advisories such as CVEs. This lack of transparency leaves users oblivious to available security updates, providing ample opportunity for attackers to exploit unpatched vulnerabilities. Consequently, identifying silent security patches just in time when they are released is essential for preventing n-day attacks, and for ensuring robust and secure maintenance practices. With LLMDA we propose to (1) leverage large language models (LLMs) to augment patch information with generated code change explanations, (2) design a representation learning approach that explores code-text alignment methodologies for feature combination, (3) implement a label-wise training with labelled instructions for guiding the embedding based on security relevance, and (4) rely on a probabilistic batch contrastive learning mechanism for building a high-precision identifier of security patches. We evaluate LLMDA on the PatchDB and SPI-DB literature datasets and show that our approach substantially improves over the state-of-the-art, notably GraphSPD by 20% in terms of F-Measure on the SPI-DB benchmark.

==> macros1.tex <==
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% black text
\newcommand\black[1]{\textcolor{black}{#1}}
\usepackage{graphicx} % For including graphics
\usepackage{caption} % For captions
\usepackage{subcaption} % For subfigures
\usepackage{natbib}
\setcitestyle{numbers,square}
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{moreverb}
\usepackage{fontenc}
\usepackage{amsmath}
\usepackage{fancybox}
\usepackage{color}
\usepackage{colortbl}
\usepackage{array}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{listings}
\usepackage{makecell}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage[multiple]{footmisc}
\usepackage{wasysym}
\usepackage{balance}
\usepackage{csvsimple}
\usepackage{longtable}
\usepackage{caption}
\usepackage{url}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{subcaption}
\usepackage{marvosym}
\usepackage{pifont}% http://ctan.org/pkg/pifont%\usepackage{subfigure}
\usepackage{courier}
\usepackage{afterpage,lipsum}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{tcolorbox}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{float}
\usepackage{soul}
\usepackage{rotating} 


\lstset{
  frame=tb,
  framerule=0.2mm,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
%   numbers=left,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  escapeinside=``,
  tabsize=4,
  extendedchars=false
}


\lstset{
    basicstyle=\ttfamily,
    mathescape, % Allows $...$ to be treated as math mode in listings
    breaklines=true, % Allows line breaking
    postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space}
}


% variable definition
\newcommand{\tang}[1]{\textcolor{blue}{Tang: }\textcolor{red}{#1}}
\newcommand{\toolname}{\emph{\sc llmda}\xspace}

\newcommand{\basicalert}[2]{\fbox{\bfseries\sffamily\scriptsize\color{blue} #1}{\sf\small$\blacktriangleright$\textit{\color{red} #2}$\blacktriangleleft$}}
\newcommand{\jk}[1]{\basicalert{Jacques}{#1}}
\newcommand{\tb}[1]{\basicalert{Bissyande}{#1}}
\newcommand{\daniel}[1]{\basicalert{From Daniel}{#1}}
\newcommand{\tian}[1]{\basicalert{From Haoye}{#1}}
\newcommand{\yw}[1]{\basicalert{From Yewei}{#1}}
\newcommand{\ah}[1]{\basicalert{From Andrew}{#1}}
\newcommand{\ak}[1]{\basicalert{From Saad}{#1}}
\newcommand{\kisub}[1]{\basicalert{From Kisub}{#1}}


\newcommand{\definition}[1]{
	\setlength{\fboxrule}{1pt}
	\begin{center}\
		\noindent\fcolorbox{black}{white!10}{
			\begin{minipage}{.92\linewidth}
				#1
			\end{minipage}
		}
	\end{center}
	\smallskip
}

\newcommand{\find}[1]{
\begin{tcolorbox}[leftrule=0.4mm,rightrule=0mm,toprule=0mm,bottomrule=0mm,left=0.0pt,right=0.0pt,top=0pt,bottom=0pt]%[tile,size=fbox,boxsep=2mm,boxrule=0pt,top=0pt,bottom=0pt,borderline={0.5mm}{0pt}{black!70!white},colback=black!5!white]
\em #1
\end{tcolorbox}
}


% \newcommand{\find}[1]{
% 	\setlength{\fboxrule}{1pt}
% 	\begin{center}\
% 		\noindent\fcolorbox{black}{gray!10}{
% 		\begin{minipage}{.92\linewidth}
% 			#1
% 		\end{minipage}
% 	}
% 	\end{center}
% 	\smallskip
% }

\pagestyle{plain}

==> sections/7.Discussion.tex <==
\section{Discussion}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/3copycopy.pdf}
    \caption{Resource Leakage}
    \label{fig:c1}
\end{figure}
PatchDB presents an extensive collection of various vulnerability types identified in software patches. Every patch in this dataset has been meticulously labeled based on the vulnerabilities it addresses. As shown in Figure~\ref{fig:patchDB_stats}, ``NULL pointer dereference" emerges as the dominant vulnerability, accounting for 70.27\% . Other significant vulnerabilities include ``buffer overflow" with 10.03\% and ``double free/use after free" at 9.62\%. The dataset doesn't neglect subtler vulnerabilities either, with instances like ``improper authentication" and ``uncontrolled resource consumption" contributing to 0.31\% and 0.07\%, respectively. Even rarer vulnerabilities such as ``race condition" and ``uninitialized use" are documented, reinforcing PatchDB's position as a comprehensive resource for examining and grasping software vulnerabilities.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/data.pdf}
    \caption{Security subtype (PatchDB) distribution (Log Scale).}
    \label{fig:patchDB_stats}
\end{figure}



In this section, we also investigate how \toolname works in real cases in different categories. To empirically assess the efficacy and interpretability of our proposed model, we meticulously selected a sample comprising 11 data entries, each representing one category from the PatchDB dataset. Central to our examination were the attributes of `patch', `explanation', and `description' in each data entry and their semantic correlation with the dichotomous labels of `security' and `non-security'. Utilizing the attention heatmap as a visualization tool, our findings delineate that, within the sampled subset, the contribution of the `patch' to the model's prediction was notably minimal. In contrast, both `explanation' and `description' demonstrated substantial and nearly equivalent influences on the predictive outcomes.

% \noindent
% \textbf{Assessing the Efficacy of {\em \toolname} across Diverse Patch Categories}

% The versatility and effectiveness of \toolname can be evaluated by its performance across various software patches. These patches, which are frequently released to address vulnerabilities, differ significantly in complexity and underlying security challenges. For our assessment, we categorized patches based on their primary function and applied \toolname to a dataset of 10,000 patches from open-source projects spanning five years. The key metrics under consideration included the detection rate of vulnerabilities post-patching, false positives generated, and the time taken for analysis.

% Our findings revealed \toolname's high proficiency in detecting buffer overflow vulnerabilities with a detection rate of 95\%. However, it also generated a slightly higher false positive rate in this category. Remarkable accuracy was observed for patches addressing race conditions, attributed to its advanced concurrency analysis module. Patches addressing improper authentication vulnerabilities were adequately detected at 85\%, but the analysis time was longer, suggesting room for optimization. As cyber threats continue to advance, refining tools like \toolname to address these nuances is essential for maintaining robust cybersecurity infrastructures.


% \begin{figure*}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/1.pdf}
%         \caption{Buffer Overflow}
%         \label{fig:c1}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/2.pdf}
%         \caption{Improper Authentication}
%         \label{fig:c2}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/3.pdf}
%         \caption{Resource Leakage}
%         \label{fig:c3}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/4.pdf}
%         \caption{Double Free or Use After Free}
%         \label{fig:c4}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/5.pdf}
%         \caption{Integer Overflow}
%         \label{fig:c5}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/6.pdf}
%         \caption{NULL Pointer Dereference}
%         \label{fig:c6}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/7.pdf}
%         \caption{Improper Input Validation}
%         \label{fig:c7}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/8.pdf}
%         \caption{Uncontrolled Resource Consumption}
%         \label{fig:c8}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/9.pdf}
%         \caption{Race Condition}
%         \label{fig:c9}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/10.pdf}
%         \caption{Uninitialized Use}
%         \label{fig:c10}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.47\linewidth}
%         \includegraphics[width=\textwidth]{figures/11.pdf}
%         \caption{Other Vulnerabilities}
%         \label{fig:c11}
%     \end{subfigure}
%     \caption{Subfigures of vulnerabilities}
%     \label{fig:subfigures}
% \end{figure*}



